Towards Perceiving Small Visual Details in Zero-shot Visual Question Answering with Multimodal LLMs

Multimodal Large Language Models (MLLMs) have recently achieved promising zero-shot accuracy on visual question answering (VQA) -- a fundamental task affecting various downstream applications and domains. Given the great potential for the broad use of these models, it is important to investigate their limitations in dealing with different image and question properties. In this work, we investigate whether MLLMs can perceive small details as well as large details in images. In particular, we show that their zero-shot accuracy in answering visual questions is very sensitive to the size of the visual subject of the question, declining up to 46% with size. Furthermore, we show that this effect is causal by observing that human visual cropping can significantly mitigate their sensitivity to size. Inspired by the usefulness of human cropping, we then propose five automatic visual cropping methods -- leveraging either external localization models or the decision process of the given MLLM itself -- as inference time mechanisms to improve the zero-shot performance of MLLMs. We study their effectiveness on four popular VQA datasets, and a subset of the VQAv2 dataset tailored towards fine visual details. Our findings suggest that MLLMs should be used with caution in detail-sensitive VQA applications, and that visual cropping is a promising direction to improve their zero-shot performance. To facilitate further investigation of MLLMs' behaviors, our code and data are publicly released.

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sections/4_cas_grad.tex <==
\section{Native \vc{}}
\label{sec:native}

The visual cropping methods we introduced in \autoref{sec:off the shelf} use off-the-shelf pretrained models which bring in external knowledge, therefore it is unclear whether these methods help the MLLM better understand the question -- know where to look in the image -- or better perceive small visual details -- solving the limitation we observed in~\autoref{sec:human_crop}. To address this ambiguity and dig more into the decision-making process of MLLMs, in this section, we propose two visual cropping methods that natively utilize the MLLM's inference time gradients and attention maps for finding the region of interest in images. Performance gain from these methods would show to what extent the MLLM itself knows `where to look' but fails to perceive small details.



\subsection{Tracking Gradients (\grad)}
\label{sec:grad}

To see where the MLLM is trying to look in the image, \ie, the region of interest from the MLLM's own perspective, \grad~ inspects the gradient of the model's decision with respect to the image (at the pixel level) and determines the image region with the highest gradient magnitude.
To get a differentiable representation of the model's decision, we define it as the logarithm of the maximum softmax probability at the first answer position. This is represented as \( l = \log(\text{softmax}(\mathbf{Z})_{t^*}) \), where \( t^* \) is the token with the highest logit and \( \mathbf{Z} \in \mathbb{R}^{D_v}\) is the output logit of the LLM's head, with $D_v$ denoting the vocabulary size. This representation emphasizes the most relevant token, \( t^* \), while maintaining the contextual information from the entire vocabulary.
Next, we take the gradient of the loss function \( l \) with respect to the input image, \ie, \( \frac{\partial{l}}{\partial{x}} \in \mathbb{R}^{H \times W \times C} \), where \( \mathrm{x} \in \mathbb{R}^{H \times W \times C} \) represents the image with spatial dimensions \( (H, W) \) and \( C \) color channels. Since we are interested in discovering regions where changes have the strongest effect on the decision, we compute the L2-norm of the gradient across the channel dimension \( \lVert \frac{\partial{l}}{\partial{x}} \rVert_2 \in \mathbb{R}^{H \times W} \), and then aggregate over each image patch of the ViT, resulting in a matrix \( M \in \mathbb{R}^{N\times N} \) where each element of \( M \) reflects the importance of a respective image patch in changing the MLLM decision. 


\subsection{Tracking Attention Scores (\att)}
\label{sec:cas}


In the previous section, by tracking the pixel level image gradient, we looked for regions whose change caused the largest \textit{change in the model's decision}. In this section, we instead want to look for the regions whose features caused the \textit{current model's decision}. To this end, utilizing the attention scores computed inside Transformer blocks as an indication of importance, we will combine how important each image region is to each Q-former token ($A_{ti}$), with how important each Q-former token is to the model's decision ($A_{st}$). \att~ consists of three steps (\autoref{fig:cas}): 1) generation of token-to-image attention maps, 2) decision-to-token attention maps, and 3) attention score aggregation. % and explained below.

\textbf{Generating Token-to-Image Attention Maps.}
As is shown in the bottom right block of~\autoref{fig:cas}, BLIP-2 uses a frozen ViT to extract image features, which are used for cross-attention in token mapping (Q-former)~\cite{li2023blip}. In the green block of~\autoref{fig:cas}, we extract the cross-attention score through all layers of Q-former, denoted as \( A_{ti} \in \mathbb{R}^{L \times H \times T \times N^2} \), where $L, H$ are the number of layers and heads-per-layer in Q-former, respectively, $T$ is the number of query tokens of Q-former, $N^2$ denotes number of image patches from ViT. Next, we weight \( \mathrm{A_{ti}}\) with the ReLU-gated derivative of $l$ with respect to each of them, formally denoted as \( \sigma(\nabla_{A_{ti}} l) \) , which is shown by the right side cuboids. Then we average them over layers and heads. The weighting by gated gradients serves as a way to diminish attention maps that are not actually used in the final model's decision, similar to~\cite{pnpvqa, pnpvqa2, gradcam}.

\textbf{Generating Decision-to-Token Attention Maps.}
The outputs of the Q-former serve as soft embeddings for the LLM, which conditions the predictions on the soft embeddings and the question. In order to measure the importance of each vision-based soft embedding in answering the question, we extract the cross-attention scores (encoder-decoder architecture) or self-attention scores (decoder-only architecture), resulting in \( \mathrm{A_{st}} \in \mathbb{R}^{L \times H \times S \times T} \), which is shown by~\autoref{fig:cas} blue block, where $S$ is the number of tokens where we track the $l$, defined in~\autoref{sec:grad}, which is 1 according to our definition of model's decision. We apply the same defined ReLU-gated derivative score \( \sigma(\nabla_{A_{st}} l) \) to  \( \mathrm{A_{st}} \), and average them over layers and heads.

\textbf{Attention Score Aggregation.}
The final importance map is the matrix multiplication between the two weighted attention maps (white block in~\autoref{fig:cas}), resulting in \( M \in \mathbb{R}^{N \times N}\), indicating how important each image token is to model's decision. 

\subsection{Postprocessing and Cropping}
\label{sec:ppc}

Both of the~\att~and~\grad~techniques result in an importance map \( M \in \mathbb{R}^{N \times N}\). In this section, we will describe how we convert $M$ to the final bounding box.


\textbf{Filtering Out Non-Edge Area.}
Typically, edges inside of images often contain critical information, characterized by noticeable color variations among adjacent pixels. We note that gradient values and attention scores include redundant data in non-edge areas, such as white skies. To mitigate this, we employ a high-pass filter with a kernel size of \(K_h\), specifically designed to exclude these less informative regions. Subsequently, a median filter with a kernel size of \(K_m\) is applied to reduce salt-and-pepper noise.  This filtered map is then patched to align with $M$'s dimensions and is utilized to assign weights within $M$, resulting in $M'$: an updated map that prioritizes areas with significant edge information. The whole procedure is illustrated in the left part of \autoref{fig:connect}.


\textbf{Bounding Box Selection.}
Given the resulting score map $M'$ and the set of image patches \( P \), we select a specific subset \(P^{(k)} \subset P\), which constitutes \( K \) patches in \( P \), maximizing \( \sum_{x \in P^{(k)}} M_{x} \), where \( M'_{x} \) denotes the score of each patch \( x \) in the subset \( P^{(k)} \).
Subsequently, all patches not included in \( P^{(k)} \) are assigned a value of zero. As is depicted in right part of~\autoref{fig:connect}, among \(P^{(k)}\), we identify all of the connected components regardless of the values of the patches.\footnote{We define connectivity in all eight possible directions: the four cardinal directions (up, down, left, and right) and the four diagonal directions.} Finally, we select the connected component with the highest cumulative score inside (blue one in~\autoref{fig:connect}). The smallest rectangle enclosing this selected component is selected as the final bounding box.

==> sections/4_outsidemodel.tex <==
\section{\vc{} with External Knowledge}
\label{sec:off the shelf}
The accuracy gain achieved by human visual cropping in~\autoref{sec:human_crop} shows the potential benefit of zooming in towards the relevant region of the input image for improving the accuracy of the zero-shot VQA models. To realize this potential in practice, in this section, we define automatic visual cropping methods, illustrated in~\autoref{fig:methods}, whose goal is to find the approximate region of interest in images, \ie, the region containing the subject of a question, and then to zoom into that region via visual cropping.

\textbf{\clip.} The intuition of this method is to progressively refine the image towards the region of highest relevance to a given question using CLIP~\cite{clip}. CLIP consists of an image encoder and a text encoder, which are trained on a large dataset of image-caption pairs to map each image (caption) close to its caption (image) and far from all other captions (images). The result is an aligned shared space where various images can be directly compared with various texts in terms of relevance. To find the region of interest, given an image-question pair, we first crop the image from the four sides (top, bottom, left, and right) at a cropping ratio of 0.9 to produce four overlapping cropped images. We then use CLIP to assess the semantic similarity between these cropped images and the question. The highest-scoring crop is chosen as the input for the next iteration. This process is repeated for 20 iterations, and the cropped image with the highest CLIP similarity to the question is selected.

\textbf{\yolo.} Instead of a progressive approach to finding the region of interest, in this method we select candidate regions based on a state-of-the-art object detection method: YOLOv8~\citep{Jocher_YOLO_by_Ultralytics_2023} pretrained on COCO~\cite{lin2014mscoco}. Using YOLO, we filter out regions that contain no salient objects -- \ie, regions for which CLIP could mistakenly assign high similarity. More concretely, for each question-image pair, we first use YOLO to collect bounding boxes for all predicted objects with confidence higher than 0.25 (the recommended default).\footnote{https://docs.ultralytics.com/modes/predict} Then, for each predicted bounding box, we crop its corresponding image and compute its similarity to the question using CLIP. Finally, the bounding box with the highest similarity score is selected as the region of interest.

\textbf{\sam.} A limitation of YOLO is that it only provides bounding boxes corresponding to a fixed number of object classes. To overcome this issue, we use the segment anything model (SAM)~\cite{kirillov2023segment}, which has shown state-of-the-art zero-shot segmentation performance. SAM can provide an extensive set of segmentation masks for each image, thus providing a more granular set of salient candidate regions compared to YOLO. More concretely, for each image-question pair, we feed the image into SAM, which provides an extensive set of segmentation masks corresponding to all objects and object parts. Then, we translate these masks into bounding boxes by computing the smallest bounding box that covers each segmentation mask. Finally, similar to \yolo, we select the bounding box with the highest CLIP similarity to the question as the region of interest.

One drawback of visual cropping is that some questions might need to have a global view of the image. To address this issue, we directly extend the original image tokens by \textbf{concatenating} the visually cropped image tokens, as illustrated in~\autoref{fig:methods}. This concatenation utilizes the fact that MLLMs typically convert the image into a series of tokens. We use this image token concatenation when applying the visual cropping methods to BLIP-2 models. In the next section, we will investigate the effectiveness of the proposed methods for improving the accuracy of zero-shot VQA models.
